AutoKaggle: A Multi-Agent Framework for Autonomous Data Science Competitions

Data science tasks involving tabular data present complex challenges that require sophisticated problem-solving approaches. We propose AutoKaggle, a powerful and user-centric framework that assists data scientists in completing daily data pipelines through a collaborative multi-agent system. AutoKaggle implements an iterative development process that combines code execution, debugging, and comprehensive unit testing to ensure code correctness and logic consistency. The framework offers highly customizable workflows, allowing users to intervene at each phase, thus integrating automated intelligence with human expertise. Our universal data science toolkit, comprising validated functions for data cleaning, feature engineering, and modeling, forms the foundation of this solution, enhancing productivity by streamlining common tasks. We selected 8 Kaggle competitions to simulate data processing workflows in real-world application scenarios. Evaluation results demonstrate that AutoKaggle achieves a validation submission rate of 0.85 and a comprehensive score of 0.82 in typical data science pipelines, fully proving its effectiveness and practicality in handling complex data science tasks.

==> tables/table_ablation_debugging_times.tex <==
\begin{table*}[t]
\caption{Performance metrics across different debugging times. Evaluated with completion rate, average normalized performance score, best normalized performance score, and comprehensive score. Best performance scores are underlined. DT refers to debugging times.}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lp{2.0cm}c c c cc@{}}
\toprule
 % & & \textbf{\space Titanic \space} & \textbf{House Prices \space} & \textbf{Spaceship Titanic \space} & \textbf{Academic Success \space} & \textbf{Avg.} \\ \midrule
  & & \textbf{Titanic} & \textbf{House Prices} & \textbf{Spaceship Titianic} & \textbf{Academic Success} & \textbf{Avg.} \\ \midrule
\multirow{4}{*}{\textbf{CR (\%)}} 
& \textbf{\space\space\space DT = 0} & 20.0 & 0 & 0 & 0 & 5.0 \\
& \textbf{\space\space\space DT = 5} & 80.0 & 40.0 & 40.0 & 40.0 & 50.0 \\
& \textbf{\space\space\space DT = 10} & 80.0 & 60.0 & 60.0 & 60.0 & 65.0 \\
& \textbf{\space\space\space DT = 15} & \underline{100.0} & \underline{80.0} & \underline{80.0} & \underline{80.0} & \underline{85.0} \\ [2pt]\hdashline\\[-8pt]

\multirow{4}{*}{\textbf{CS}} 
& \textbf{\space\space\space DT = 0} & 0.482 & 0 & 0 & 0 & 0.120 \\
& \textbf{\space\space\space DT = 5} & 0.790 & 0.628 & 0.587 & 0.610 & 0.654 \\
& \textbf{\space\space\space DT = 10} & 0.790 & 0.728 & 0.691 & 0.709 & 0.730 \\
& \textbf{\space\space\space DT = 15} & \underline{0.888} & \underline{0.831} & \underline{0.786} & \underline{0.810} & \underline{0.829} \\ [2pt]\hdashline\\[-8pt]

\multirow{4}{*}{\textbf{BNPS}} 
& \textbf{\space\space\space DT = 0} & 0.763 & 0 & 0 & 0 & 0.191 \\
& \textbf{\space\space\space DT = 5} & 0.787 & 0.867 & 0.785 & 0.829 & 0.817 \\
& \textbf{\space\space\space DT = 10} & 0.787 & 0.867 & 0.801 & 0.829 & 0.821 \\
& \textbf{\space\space\space DT = 15} & \underline{0.787} & \underline{0.880} & \underline{0.801} & \underline{0.829} & \underline{0.824} \\  

\bottomrule
\end{tabular}}    
\end{center}
\label{tab:ablation_debugging_times}
\vspace{-5pt}
\end{table*}


==> tables/table_fe_debugging_times.tex <==
\begin{table*}[t]
\caption{Total debugging times of five trials in feature engineering phase.}
\begin{center}
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{@{}lc c c c@{}}
\toprule
 & \textbf{\space Titanic} & \textbf{\space House Prices} & \textbf{\space Spaceship Titanic} & \textbf{\space Academic Success \space} \\ \midrule
\textbf{DC Tools} & 2 & 24 & 21 & 15 \\ 
\textbf{DC \& FE Tools} & 8 & 36 & 33 & 32 \\ 
\bottomrule
\end{tabular}}    
\end{center}
\label{tab:fe_debugging_times}
\vspace{-5pt}
\end{table*}

